Some inequalities for tetrahedra

We prove inequalities involving intrinsic and extrinsic radii and diameters of tetrahedra.

==> Macros.tex <==
% V 4.0
\newcommand{\nc}{\newcommand}
\newcommand{\df}{\def}
\RequirePackage{ifthen}
\RequirePackage{xcolor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%COLABORATING TOOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\EnableColaboratingTools -- no comment
%\DisableColaboratingTools -- no comment
%\begin{CTbox}[title]  ... box content ... \end{WB} -- Inline box
%\CTnote{text note} -- margin note displayed if C.T. enabled
%\CTemph[color]{emphasized text} -- Chng color iff C.T. are enable
%\CTewn[color]{emphasized text}{note} --  Emphasis with Note
%\CTrep[Comment]{new text}{old text} -- Text replacement

%\CTdnote,\CTdewn,\CTdrep are delayed version of the same command without "d"
%The margin notes are displayed at the next \CTprintnotes.
%(usefull because non delayed version does not works in several environments)

%\CTcolorbox{color} -- color of boxes
%\CTcoloremph{color} --color of ephasis
%\CTcolrep{new text color}{old text color} -- colors of replacements
%\CTcolnote{color} -- color of notes and replacements comments

%\CTsetnotewidth{width}

\makeatletter
\newcommand{\Working@Stuff@Flag}{0}
%\newlength{\WS@Dummy@Length}
\newlength{\CT@margpar@len}
\setlength{\CT@margpar@len}{3.2cm}
%%default colors
\definecolor{CT@color@emph}{rgb}{0,0,.8}
\definecolor{CT@color@box}{rgb}{0,0,.8}
\definecolor{CT@color@rep@nt}{rgb}{0,.5,0}
\definecolor{CT@color@rep@ot}{rgb}{.8,0,0}
\definecolor{CT@color@note}{rgb}{.5,0,.5}


\newcommand{\CTcolorbox}[1]{\colorlet{CT@color@box}{#1}}
\newcommand{\CTcoloremph}[1]{\colorlet{CT@color@emph}{#1}}
\newcommand{\CTcolornote}[1]{\colorlet{CT@color@note}{#1}}
\newcommand{\CTcolorrep}[2]{\colorlet{CT@color@rep@nt}{#1}\colorlet{CT@color@rep@ot}{#2}}
\newcommand{\CTsetnotewidth}[1]{\setlength{\CT@margpar@len}{#1}}

\newcommand{\EnableColaboratingTools}{\renewcommand{\Working@Stuff@Flag}{1}}
\newcommand{\DisableColaboratingTools}{\renewcommand{\Working@Stuff@Flag}{0}}

%%boxes
\newlength{\WS@Dummy@Length}
\newenvironment{CTbox}[1][]
{\color{CT@color@box}

 \if\Working@Stuff@Flag1\begin{tabular}{|p{0.9\textwidth}|}
 \hline\\
 \ifx\relax#1\relax
 \else
 \hfill{\bf #1}\hfill\rule{-.01pt}{0pt}\\
 \hline
 \fi
 \else
 \settowidth{\WS@Dummy@Length}\bgroup
  \fi
}
{\if\Working@Stuff@Flag1\\ \hline
 \end{tabular}
 \else
 \egroup%
 \fi
 
}

%dnotes
\gdef\CT@ns@index{CT@note@stack}

\newcounter{CT@counter@dn}
\newcounter{CT@counter@save}
\newcounter{CT@counter}
\setcounter{CT@counter}{1}


\newcommand{\CT@note@Label}[1]{{%
\color{CT@color@note}%
\ensuremath{\color{CT@color@note}\rule{0pt}{1ex}^{\text{\roman{#1}}}}%
}}
 
\newcommand{\CTdnote}[1]{{%
\if\Working@Stuff@Flag1%
\CT@note@Label{CT@counter}%
\expandafter\gdef\csname\CT@ns@index\endcsname{#1}%
\xdef\CT@ns@index{@\CT@ns@index}%
\if0\arabic{CT@counter@dn}%
\setcounter{CT@counter@save}{\value{CT@counter}}%
\fi%
\stepcounter{CT@counter@dn}%
\stepcounter{CT@counter}%
\fi%
}}
%%%printnotes

\newcommand{\CT@printnotes}{%
\if0\arabic{CT@counter@dn}%
\else%
{\color{CT@color@note}%
\fbox{\parbox{\CT@margpar@len}{%
\CT@note@Label{CT@counter@save}%
\stepcounter{CT@counter@save}%
\csname\CT@ns@index\endcsname%
}}%
\if1\arabic{CT@counter@dn}\else\\ \fi%
}%
\xdef\CT@ns@index{@\CT@ns@index}%
\addtocounter{CT@counter@dn}{-1}%
\CT@printnotes%
\fi%
}

\newcommand{\CTprintnotes}{%
\xdef\CT@ns@index{CT@note@stack}%
\marginpar{\CT@printnotes}%
\xdef\CT@ns@index{CT@note@stack}%
}

%%CTnote 
\nc{\CTnote}[1]{%
\if\Working@Stuff@Flag1%
\CTdnote{#1}%
\CTprintnotes%
\fi%
} 
%%CTemph
 
\newcommand{\CTemph}[2][CT@color@emph]{%
{\if\Working@Stuff@Flag1%
\color{#1}%
\fi%
#2}%
}% 

%%ewn 
\newcommand{\CTdewn}[3][CT@color@emph]%
{\CTemph[#1]{#2}%
\CTdnote{#3}%
} 
\newcommand{\CTewn}[3][CT@color@emph]%
{\CTemph[#1]{#2}%
\CTnote{#3}%
} 
%%rep
\newcommand{\CTrep}[3][]{%
\CTdrep[#1]{#2}{#3}%
\CTprintnotes%
}

\newcommand{\CTdrep}[3][]{%
\CTdewn[CT@color@rep@nt]{#2}%
{\if\relax#1\relax\else{\color{CT@color@note}#1}\\ \fi%
{\bf old text: }%
{\color{CT@color@rep@ot}#3}%
}%
}

 
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%racourciss divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\df\ie#1{{\mbox{{\it i.\hspace{0.06em}e.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}
\df\eg#1{{\mbox{{\it e.\hspace{0.06em}g.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citations dans Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\cit}[2][]{\ifthenelse{\equal{#1}{}}{{\rm \cite{#2}}}{{\rm \cite[#1]{#2}}}}

\makeatletter

%%%%%%%%%TURNED-M

\newcommand{\most@textstyle}{\hspace{.07em plus .01 em minus .01em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{-.315 em}\wedge\hspace{-.315 em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{.15em plus .05em minus .05em}}

\newcommand{\most@scriptstyle}{\hspace{.05705em plus .00815 em minus .00815em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{-.07 em}\wedge\hspace{-.07 em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{.12225em plus .04075em minus .04075em}}

\newcommand{\most@scriptscriptstyle}{\hspace{.05075em plus .00725 em minus .00725em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{-.063 em}\wedge\hspace{-.065 em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{.10875em plus .03625em minus .03625em}}

\newcommand{\most}{\mathchoice{\most@textstyle}{\most@textstyle}{\most@scriptstyle}{\most@scriptscriptstyle}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gestions des {|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% usage:  \set(: xyz\in XYZ | xyz is something :) 
%
%Note: \set[xx](: ...| ...:) is for backward compatibility, xx is ignored.
%Note: \seti is an alias of \set, still for backward compatibility
%Note: If set are nested, inner sets must be enclosed in braces: {\set(:...|...:)}


\newlength{\Set@LH}
\newlength{\Set@RH}
\newlength{\Set@LD}
\newlength{\Set@RD}
\newlength{\Set@NoPar@W}

\newsavebox{\Set@Box@R}
\newsavebox{\Set@Box@L}

\newcommand{\Set@@}[3]{%#3=math style
\sbox{\Set@Box@L}{\ensuremath{#3#1}}
\sbox{\Set@Box@R}{\ensuremath{#3#2}}
\settoheight{\Set@LH}{\usebox{\Set@Box@L}}
\settodepth {\Set@LD}{\usebox{\Set@Box@L}}
\settoheight{\Set@RH}{\usebox{\Set@Box@R}}
\settodepth {\Set@RD}{\usebox{\Set@Box@R}}
\addtolength{\Set@LH}{\Set@LD}
\addtolength{\Set@RH}{\Set@RD}
{\def\mt{\rule[-\Set@LD]{0pt}{\Set@LH}\rule[-\Set@RD]{0pt}{\Set@RH}}
\settowidth{\Set@NoPar@W}{\ensuremath{#3\left.\mt\right.}}
\left\{\usebox{\Set@Box@L}\mt\right.\hspace{-.3\Set@NoPar@W}\left\vert\usebox{\Set@Box@R}\mt\right\}}
}


\def\Set@Smile(:#1|#2:){\mathchoice
{\Set@@{#1}{#2}{\displaystyle}}
{\Set@@{#1}{#2}{\textstyle}}
{\Set@@{#1}{#2}{\scriptstyle}}
{\Set@@{#1}{#2}{\scriptscriptstyle}}
}

\newcommand{\set}[1][]{\Set@Smile}
\newcommand{\seti}{\set}




\makeatother


